A Sample-Level Evaluation and Generative Framework for Model Inversion Attacks

Model Inversion (MI) attacks, which reconstruct the training dataset of neural networks, pose significant privacy concerns in machine learning. Recent MI attacks have managed to reconstruct realistic label-level private data, such as the general appearance of a target person from all training images labeled on him. Beyond label-level privacy, in this paper we show sample-level privacy, the private information of a single target sample, is also important but under-explored in the MI literature due to the limitations of existing evaluation metrics. To address this gap, this study introduces a novel metric tailored for training-sample analysis, namely, the Diversity and Distance Composite Score (DDCS), which evaluates the reconstruction fidelity of each training sample by encompassing various MI attack attributes. This, in turn, enhances the precision of sample-level privacy assessments. Leveraging DDCS as a new evaluative lens, we observe that many training samples remain resilient against even the most advanced MI attack. As such, we further propose a transfer learning framework that augments the generative capabilities of MI attackers through the integration of entropy loss and natural gradient descent. Extensive experiments verify the effectiveness of our framework on improving state-of-the-art MI attacks over various metrics including DDCS, coverage and FID. Finally, we demonstrate that DDCS can also be useful for MI defense, by identifying samples susceptible to MI attacks in an unsupervised manner.

==> sec/2_related.tex <==
\section{Related Work}
\label{related}
\textbf{MI attacks with DCGAN.}\quad MI attacks are broadly classified into black-box and white-box categories based on the attacker's access to the target neural network's parameters.
Initial white-box MI attacks~\cite{mi15} lacked stringent optimization constraints, leading to the generation of blurred and unrealistic samples.
To enhance sample realism, \cite{gmi20cvpr} integrated DCGAN into the MI attack framework by optimizing the latent codes of generated samples.
The use of explainable artificial intelligence tools in MI attacks was explored by \cite{xai21iccv}, while KEDMI~\cite{kedmi21iccv} advanced the field by developing an inversion-specific DCGAN featuring a multi-task discriminator and entropy loss.
Further study~\cite{rethink23cvpr} suggests improved optimization objective and model augmentation to mitigate the sub-optimum and overfitting problem.

\noindent
\textbf{MI attacks with StyleGAN.}\quad Our work primarily investigates MI inversions utilizing StyleGAN~\cite{stylegan2_20cvpr}, recognized for setting the benchmark in generating image priors for MI attacks.
\cite{vmi21nips} approached MI attacks through a probabilistic lens, employing StyleGAN to elevate image quality.
The study by \cite{mirror22ndss} introduced heuristic improvements for StyleGAN-based MI attacks in both white-box and black-box scenarios.
To overcome challenges like vanishing gradients and distributional shifts, the Plug \& Play Attack~\cite{ppa22icml} was proposed, incorporating Poincar\'e loss and a transformation-based selection mechanism.
Enhancements to this method were later made by \cite{mi23mm}, leveraging historically learned knowledge.

\noindent
\textbf{Black-box MI attacks.}\quad In the context of black-box MI attacks, where the attacker lacks access to the target model's parameters, \cite{blackbox19ccs} developed a surrogate neural network to invert the undisclosed victim model. The introduction of boundary repulsion by \cite{blackbox22cvpr} enabled MI attacks to function using only the label outputs of the victim model. Further strengthening of black-box MI attacks was achieved by \cite{blackbox23tdsc} through the integration of semantic loss regularization and adversarial example injection. The study by \cite{mi23iccvw} addressed the challenge of attacking black-box face recognition models by harnessing the stochastic properties of the denoising diffusion process from diffusion models.

\noindent
\textbf{Gradient inversion attacks.}\quad Gradient Inversion (GI)~\cite{wr1} is fundamentally different from MI attacks, where GI is concentrated on those scenarios in federated learning requiring gradient information. Notably, recent works on GI~\cite{wr2, wr3, wr4, wr6} still inherit the same evaluation metrics from previous MI works, which makes our work unique. Specifically, \cite{wr1} relaxes the strong assumption about the GI attacks and proposes a more practical scenario. Other works~\cite{wr2, wr3, wr4, wr6} propose GI attacks in FL using DCGAN and BigGAN and are assessed with basic accuracy and distance metrics as the evaluation metrics.
